Sulfur Chemistry in L1157-B1

The main carrier of sulfur in dense clouds, where it is depleted from the gas phase, remains a mystery. Shock waves in young molecular outflows disrupt the ice mantles and allow us to directly probe the material that is ejected into the gas phase. A comprehensive study of sulfur-bearing species towards L1157-B1, a shocked region along a protostellar outflow, has been carried out as part of the IRAM-30m large program ASAI. The dataset contains over 100 lines of CCS, H$_2$CS, OCS, SO, SO$_2$ and isotopologues. The results of these observations are presented, complementing previous studies of sulfur-bearing species in the region. The column densities and fractional abundances of these species are measured and together these species account for 10\% of the cosmic sulfur abundance in the region. The gas properties derived from the observations are also presented, demonstrating that sulfur bearing species trace a wide range of different gas conditions in the region.

==> linetables.tex <==
\begin{table*}
\caption{Line properties of detected transitions including: upper state energy (E$_u$); Einstein coefficients (A$_{ij}$); beam size ($\Theta_{MB}$); the peak antenna temperature with the spectrum rms in brackets; the peak, minimum and maximum velocities of the spectra, the velocity resolution, the forward and beam efficiencies, the filling factor ($\eta_{ff}$), and integrated emission ($\int T_{MB} dv$) measured in the moderate velocity regime discussed in Section~\ref{sec:lineprops}.}
\begin{tabular}{cccccccccccc}
\hline
 \textbf{Freq} & \textbf{Transition} & \boldmath$\mathrm{E_u}$  & \boldmath$\mathrm{log(A_{ij})}$ & \boldmath$\mathrm{\Theta_{MB}}$ & \boldmath$\mathrm{T_{A*,peak}}$ & \boldmath$\mathrm{V_{peak}}$ & \boldmath$\mathrm{V_{min}/V_{max}}$ &  \boldmath$\mathrm{\Delta V}$ & \boldmath$\mathrm{F_{eff}/B_{eff}}$ & \boldmath$\mathrm{\eta_{ff}}$ & \boldmath$\mathrm{\int T_{MB} dv}$ \\ 
 \textbf{GHz} & & \textbf{K} & & \textbf{\si{\arcsecond}} & \textbf{mK} &\textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & & & \textbf{K km s$^{-1}$} \\ 
\hline 
 &&&&&\textbf{CCS}&&\\ 
 \hline 
81.505 &N=6-5,J=7-6 & 15.4 & -4.61 & 30 & 33 (2) & -0.3 & -6.0/2.6 & 1.4 & 1.0& 0.3& 0.19 (0.04) \\ 
90.686 &N=7-6,J=7-6 & 26.1 & -4.48 & 27 & 11 (2) & 0.0 & -2.6/2.6 & 1.3 & 1.2& 0.3& 0.08 (0.02) \\ 
93.870 &N=7-6,J=8-7 & 19.9 & -4.42 & 26 & 31 (1) & 0.1 & -4.9/2.6 & 1.2 & 1.2& 0.4& 0.20 (0.04) \\ 
99.866 &N=8-7,J=7-6 & 28.1 & -4.35 & 25 & 11 (1) & -0.9 & -3.3/1.4 & 1.2 & 1.2& 0.4& 0.07 (0.02) \\ 
103.640 &N=8-7,J=8-7 & 31.1 & -4.30 & 24 & 10 (3) & -0.8 & -0.8/2.6 & 1.1 & 1.2& 0.4& 0.09 (0.02) \\ 
106.347 &N=8-7,J=9-8 & 25.0 & -4.25 & 23 & 31 (2) & 0.4 & -5.1/2.6 & 1.1 & 1.2& 0.4& 0.20 (0.04) \\ 
113.410 &N=9-8,J=8-7 & 33.6 & -4.18 & 22 & 16 (2) & 0.5 & -2.6/1.6 & 1.0 & 1.2& 0.5& 0.09 (0.02) \\ 
131.551 &N=10-9,J=11-10 & 37.0 & -3.97 & 19 & 24 (4) & -0.1 & -1.0/1.7 & 0.9 & 1.2& 0.5& 0.13 (0.03) \\ 
142.501 &N=11-10,J=11-10 & 49.7 & -3.87 & 17 & 16 (4) & 0.1 & 0.1/1.0 & 0.8 & 1.2& 0.6& 0.11 (0.02) \\ 
144.244 &N=11-10,J=12-11 & 43.9 & -3.85 & 17 & 21 (4) & -1.4 & -2.3/1.8 & 0.8 & 1.2& 0.6& 0.16 (0.03) \\ 
156.981 &N=12-11,J=13-12 & 51.5 & -3.74 & 16 & 25 (5) & -1.1 & -2.6/1.9 & 0.7 & 1.3& 0.6& 0.19 (0.04) \\ 
166.662 &N=13-12,J=12-11 & 61.8 & -3.66 & 15 & 24 (5) & -0.2 & -0.9/0.5 & 0.7 & 1.3& 0.7& 0.11 (0.02) \\ 
\hline 
 &&&&&\textbf{O-H$_2$CS}&&\\ 
 \hline 
104.617 &3(1,2)-2(1,1) & 23.2 & -4.86 & 24 & 85 (2) & -0.8 & -7.5/4.8 & 1.1 & 1.2& 0.4& 0.72 (0.14) \\ 
135.298 &4(1,4)-3(1,3) & 29.4 & -4.49 & 18 & 112 (3) & 0.0 & -6.9/3.5 & 0.9 & 1.2& 0.6& 0.89 (0.18) \\ 
169.114 &5(1,5)-4(1,4) & 37.5 & -4.18 & 15 & 122 (5) & -0.9 & -5.7/3.3 & 0.7 & 1.3& 0.7& 1.07 (0.21) \\ 
209.200 &6(1,5)-5(1,4) & 48.3 & -3.89 & 12 & 76 (3) & -0.8 & -6.4/2.6 & 1.1 & 1.5& 0.7& 0.74 (0.15) \\ 
244.048 &7(1,6)-6(1,5) & 60.0 & -3.68 & 10 & 58 (3) & -1.2 & -7.0/3.6 & 1.0 & 1.6& 0.8& 0.63 (0.13) \\ 
270.521 &8(1,8)-7(1,7) & 71.6 & -3.54 & 9 & 39 (5) & -1.4 & -3.6/3.0 & 2.2 & 1.7& 0.8& 0.61 (0.12) \\ 
278.887 &8(1,7)-7(1,6) & 73.4 & -3.50 & 9 & 30 (4) & -1.3 & -3.5/0.8 & 2.1 & 1.8& 0.8& 0.41 (0.08) \\ 
\hline 
 &&&&&\textbf{P-H$_2$CS}&&\\ 
 \hline 
103.051 &3(2,1)-2(2,0) & 62.6 & -5.08 & 24 & 10 (2) & 0.3 & -3.1/0.3 & 1.1 & 1.2& 0.4& 0.07 (0.02) \\ 
137.382 &4(2,3)-3(2,2) & 69.2 & -4.56 & 18 & 18 (5) & -0.8 & -1.7/-0.8 & 0.8 & 1.2& 0.6& 0.15 (0.03) \\ 
171.688 &5(0,5)-4(0,4) & 24.7 & -4.14 & 14 & 69 (8) & -0.8 & -4.2/1.2 & 0.7 & 1.3& 0.7& 0.47 (0.10) \\ 
205.987 &6(0,6)-5(0,5) & 34.6 & -3.89 & 12 & 39 (3) & 0.3 & -5.4/2.6 & 1.1 & 1.5& 0.7& 0.40 (0.08) \\ 
206.158 &6(2,4)-5(2,3) & 87.3 & -3.95 & 12 & 21 (4) & -1.9 & -3.1/1.5 & 1.1 & 1.5& 0.7& 0.20 (0.04) \\ 
240.382 &7(2,6)-6(2,5) & 98.9 & -3.73 & 10 & 13 (3) & 0.7 & 0.7/1.6 & 1.0 & 1.6& 0.8& 0.12 (0.03) \\ 
240.549 &7(2,5)-6(2,4) & 98.9 & -3.73 & 10 & 18 (3) & -1.3 & -3.2/2.6 & 1.0 & 1.6& 0.8& 0.19 (0.04) \\ 
\hline 
 &&&&&\textbf{OCS}&&\\ 
 \hline 
85.139 &7-6 & 16.3 & -5.77 & 29 & 32 (1) & -0.1 & -7.0/4.0 & 1.4 & 1.2& 0.3& 0.26 (0.05) \\ 
97.301 &8-7 & 21.0 & -5.59 & 25 & 37 (1) & 0.2 & -5.8/3.8 & 1.2 & 1.2& 0.4& 0.31 (0.06) \\ 
109.463 &9-8 & 26.3 & -5.43 & 22 & 45 (1) & 0.5 & -6.0/3.7 & 1.1 & 1.2& 0.4& 0.35 (0.07) \\ 
133.785 &11-10 & 38.5 & -5.17 & 18 & 45 (4) & 0.8 & -5.3/2.6 & 0.9 & 1.2& 0.5& 0.35 (0.07) \\ 
145.946 &12-11 & 45.5 & -5.05 & 17 & 51 (3) & 0.2 & -6.2/3.4 & 0.8 & 1.3& 0.6& 0.45 (0.09) \\ 
158.107 &13-12 & 53.1 & -4.95 & 16 & 66 (5) & 1.1 & -4.8/2.6 & 0.7 & 1.3& 0.6& 0.52 (0.10) \\ 
170.267 &14-13 & 61.3 & -4.85 & 14 & 64 (6) & 1.9 & -5.0/3.3 & 0.7 & 1.3& 0.7& 0.54 (0.11) \\ 
206.745 &17-16 & 89.3 & -4.59 & 12 & 44 (2) & 1.5 & -5.3/2.6 & 1.1 & 1.5& 0.7& 0.45 (0.09) \\ 
218.903 &18-17 & 99.8 & -4.52 & 11 & 43 (2) & 0.5 & -4.9/4.7 & 1.1 & 1.5& 0.8& 0.43 (0.09) \\ 
231.060 &19-18 & 110.9 & -4.45 & 11 & 34 (3) & 0.6 & -4.5/2.6 & 1.0 & 1.6& 0.8& 0.32 (0.06) \\ 
243.218 &20-19 & 122.6 & -4.38 & 10 & 33 (3) & 0.7 & -5.1/2.6 & 1.0 & 1.6& 0.8& 0.33 (0.07) \\ 
255.374 &21-20 & 134.8 & -4.32 & 10 & 28 (3) & 0.8 & -3.8/2.6 & 0.9 & 1.6& 0.8& 0.29 (0.06) \\ 
267.530 &22-21 & 147.7 & -4.25 & 9 & 21 (5) & 0.8 & -1.5/0.8 & 2.2 & 1.7& 0.8& 0.30 (0.06) \\ 
291.839 &24-23 & 175.1 & -4.14 & 8 & 20 (4) & -1.1 & -3.2/0.9 & 2.0 & 1.9& 0.8& 0.28 (0.06) \\ 
\hline
\end{tabular}
\label{table:lines}
\end{table*}


\begin{table*}
\caption{Continued line properties of detected transitions}
\begin{tabular}{cccccccccccc}
\hline
 \textbf{Freq} & \textbf{Transition} & \boldmath$\mathrm{E_u}$  & \boldmath$\mathrm{log(A_{ij})}$ & \boldmath$\mathrm{\Theta_{MB}}$ & \boldmath$\mathrm{T_{A*,peak}}$ & \boldmath$\mathrm{V_{peak}}$ & \boldmath$\mathrm{V_{min}/V_{max}}$ &  \boldmath$\mathrm{\Delta V}$ & \boldmath$\mathrm{F_{eff}/B_{eff}}$ & \boldmath$\mathrm{\eta_{ff}}$ & \boldmath$\mathrm{\int T_{MB} dv}$ \\ 
 \textbf{GHz} & & \textbf{K} & & \textbf{\si{\arcsecond}} & \textbf{mK} &\textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & & & \textbf{K km s$^{-1}$} \\ \hline 
 &&&&&\textbf{SO}&&\\ 
 \hline 
86.093 &2(2)-1(1) & 19.3 & -5.27 & 29 & 139 (1) & -0.1 & -20.5/4.0 & 1.4 & 1.2& 0.3& 1.07 (0.22) \\ 
99.299 &3(2)-2(1) & 9.2 & -4.94 & 25 & 1516 (2) & 0.2 & -21.0/5.0 & 1.2 & 1.2& 0.4& 11.31 (2.26) \\ 
100.029 &4(5)-4(4) & 38.6 & -5.96 & 25 & 14 (1) & 0.3 & -5.6/2.6 & 1.2 & 1.2& 0.4& 0.10 (0.02) \\ 
109.252 &2(3)-1(2) & 21.1 & -4.96 & 23 & 212 (2) & 0.5 & -15.6/3.7 & 1.1 & 1.2& 0.4& 1.64 (0.33) \\ 
129.138 &3(3)-2(2) & 25.5 & -4.64 & 19 & 315 (4) & 0.8 & -12.8/3.5 & 0.9 & 1.2& 0.5& 2.32 (0.46) \\ 
138.178 &4(3)-3(2) & 15.9 & -4.49 & 18 & 1873 (4) & 0.9 & -16.0/4.3 & 0.8 & 1.2& 0.6& 13.91 (2.78) \\ 
158.971 &3(4)-2(3) & 28.7 & -4.36 & 15 & 452 (5) & 1.1 & -12.8/4.1 & 0.7 & 1.3& 0.6& 3.67 (0.73) \\ 
172.181 &4(4)-3(3) & 33.8 & -4.23 & 14 & 389 (10) & 0.6 & -7.6/3.3 & 0.7 & 1.3& 0.7& 3.06 (0.61) \\ 
206.176 &4(5)-3(4) & 38.6 & -3.99 & 12 & 405 (4) & 0.3 & -14.4/3.7 & 1.1 & 1.5& 0.7& 3.97 (0.80) \\ 
215.220 &5(5)-4(4) & 44.1 & -3.91 & 11 & 404 (2) & 0.4 & -15.9/3.7 & 1.1 & 1.5& 0.8& 4.09 (0.82) \\ 
219.949 &6(5)-5(4) & 35.0 & -3.87 & 11 & 1293 (14) & 0.5 & -14.4/4.7 & 1.1 & 1.5& 0.8& 13.18 (2.64) \\ 
251.825 &5(6)-4(5) & 50.7 & -3.71 & 10 & 349 (23) & -0.2 & -5.8/2.6 & 0.9 & 1.6& 0.8& 4.01 (0.80) \\ 
258.255 &6(6)-5(5) & 56.5 & -3.67 & 10 & 246 (3) & -0.1 & -16.4/4.4 & 0.9 & 1.7& 0.8& 2.88 (0.58) \\ 
261.843 &7(6)-6(5) & 47.6 & -3.63 & 9 & 792 (4) & 0.8 & -16.2/4.4 & 0.9 & 1.7& 0.8& 8.30 (1.66) \\ 
286.340 &1(1)-1(0) & 15.2 & -4.84 & 9 & 35 (7) & 0.9 & -1.2/0.9 & 2.1 & 1.8& 0.8& 0.43 (0.09) \\ 
296.550 &6(7)-5(6) & 64.9 & -3.48 & 8 & 184 (3) & -1.0 & -19.2/3.0 & 2.0 & 1.9& 0.8& 2.69 (0.54) \\ 
301.286 &7(7)-6(6) & 71.0 & -3.46 & 8 & 105 (3) & -1.0 & -14.9/3.0 & 2.0 & 1.9& 0.9& 1.64 (0.33) \\ 
304.077 &8(7)-7(6) & 62.1 & -3.43 & 8 & 271 (6) & -0.9 & -14.8/3.0 & 2.0 & 2.0& 0.9& 4.27 (0.86) \\ 
309.502 &2(2)-2(1) & 19.3 & -4.84 & 8 & 31 (3) & 1.1 & -4.8/3.0 & 1.9 & 2.0& 0.9& 0.49 (0.10) \\ 
339.341 &3(3)-3(2) & 25.5 & -4.83 & 7 & 27 (4) & -0.5 & -4.1/1.2 & 1.8 & 2.3& 0.9& 0.45 (0.09) \\ 
340.714 &7(8)-6(7) & 81.2 & -3.29 & 7 & 122 (5) & -0.5 & -14.6/3.0 & 1.8 & 2.3& 0.9& 2.40 (0.48) \\ 
344.310 &8(8)-7(7) & 87.5 & -3.28 & 7 & 73 (8) & -0.5 & -5.7/1.3 & 1.7 & 2.4& 0.9& 1.23 (0.25) \\ 
346.528 &9(8)-8(7) & 78.8 & -3.26 & 7 & 181 (4) & -0.5 & -14.3/4.7 & 1.7 & 2.0& 0.9& 2.78 (0.56) \\ 
\hline 
 &&&&&\textbf{SO$_2$}&&\\ 
 \hline 
83.688 &8(1,7)-8(0,8) & 36.7 & -5.17 & 29 & 82 (1) & -1.6 & -14.2/2.6 & 1.4 & 1.0& 0.3& 0.54 (0.11) \\ 
104.029 &3(1,3)-2(0,2) & 7.7 & -5.00 & 24 & 157 (2) & -0.8 & -14.3/10.5 & 1.1 & 1.2& 0.4& 1.26 (0.25) \\ 
104.239 &10(1,9)-10(0,10) & 54.7 & -4.95 & 24 & 58 (1) & 0.3 & -7.5/2.6 & 1.1 & 1.2& 0.4& 0.47 (0.09) \\ 
131.014 &12(1,11)-12(0,12) & 76.4 & -4.73 & 19 & 37 (5) & -0.1 & -3.6/1.7 & 0.9 & 1.2& 0.5& 0.31 (0.06) \\ 
134.004 &8(2,6)-8(1,7) & 43.1 & -4.60 & 18 & 16 (3) & -0.9 & -4.4/0.9 & 1.7 & 1.2& 0.5& 0.14 (0.03) \\ 
135.696 &5(1,5)-4(0,4) & 15.7 & -4.66 & 18 & 245 (5) & 0.0 & -6.0/3.5 & 0.9 & 1.2& 0.6& 1.83 (0.37) \\ 
140.306 &6(2,4)-6(1,5) & 29.2 & -4.60 & 18 & 33 (4) & 0.1 & -3.2/1.8 & 0.8 & 1.2& 0.6& 0.24 (0.05) \\ 
151.378 &2(2,0)-2(1,1) & 12.6 & -4.73 & 16 & 27 (4) & 1.8 & -2.8/1.8 & 0.8 & 1.3& 0.6& 0.22 (0.04) \\ 
158.199 &3(2,2)-3(1,3) & 15.3 & -4.60 & 16 & 62 (5) & 0.4 & -4.0/1.9 & 0.7 & 1.3& 0.6& 0.41 (0.08) \\ 
160.827 &10(0,10)-9(1,9) & 49.7 & -4.40 & 15 & 251 (5) & 0.4 & -7.6/3.3 & 0.7 & 1.3& 0.6& 1.96 (0.39) \\ 
163.605 &14(1,13)-14(0,14) & 101.8 & -4.52 & 15 & 30 (6) & -1.0 & -1.7/1.2 & 0.7 & 1.3& 0.6& 0.20 (0.04) \\ 
165.144 &5(2,4)-5(1,5) & 23.6 & -4.51 & 15 & 59 (11) & 0.5 & -2.4/1.9 & 0.7 & 1.3& 0.6& 0.47 (0.10) \\ 
165.225 &7(1,7)-6(0,6) & 27.1 & -4.38 & 15 & 278 (6) & 0.5 & -7.3/3.3 & 0.7 & 1.3& 0.6& 2.25 (0.45) \\ 
200.809 &16(1,15)-16(0,16) & 130.7 & -4.33 & 12 & 11 (2) & -0.9 & -0.9/0.3 & 1.2 & 1.5& 0.7& 0.07 (0.01) \\ 
203.391 &12(0,12)-11(1,11) & 70.1 & -4.06 & 12 & 147 (3) & 0.3 & -12.4/14.1 & 1.1 & 1.5& 0.7& 1.50 (0.30) \\ 
205.300 &11(2,10)-11(1,11) & 70.2 & -4.27 & 12 & 21 (3) & -0.8 & -3.1/2.6 & 1.1 & 1.5& 0.7& 0.21 (0.04) \\ 
208.700 &3(2,2)-2(1,1) & 15.3 & -4.17 & 12 & 90 (3) & 0.4 & -6.4/3.7 & 1.1 & 1.5& 0.7& 0.81 (0.16) \\ 
221.965 &11(1,11)-10(0,10) & 60.4 & -3.94 & 11 & 150 (2) & -0.6 & -13.2/3.7 & 1.1 & 1.5& 0.8& 1.60 (0.32) \\ 
225.153 &13(2,12)-13(1,13) & 93.0 & -4.19 & 11 & 13 (2) & -0.5 & -3.6/1.6 & 1.0 & 1.5& 0.8& 0.14 (0.03) \\ 
235.151 &4(2,2)-3(1,3) & 19.0 & -4.11 & 10 & 83 (3) & -0.4 & -6.4/2.6 & 1.0 & 1.6& 0.8& 0.82 (0.16) \\ 
\hline
\end{tabular}
\label{table:lines2}
\end{table*}


\begin{table*}
\caption{Continued line properties of detected transitions}
\begin{tabular}{cccccccccccc}
\hline
 \textbf{Freq} & \textbf{Transition} & \boldmath$\mathrm{E_u}$  & \boldmath$\mathrm{log(A_{ij})}$ & \boldmath$\mathrm{\Theta_{MB}}$ & \boldmath$\mathrm{T_{A*,peak}}$ & \boldmath$\mathrm{V_{peak}}$ & \boldmath$\mathrm{V_{min}/V_{max}}$ &  \boldmath$\mathrm{\Delta V}$ & \boldmath$\mathrm{F_{eff}/B_{eff}}$ & \boldmath$\mathrm{\eta_{ff}}$ & \boldmath$\mathrm{\int T_{MB} dv}$ \\ 
 \textbf{GHz} & & \textbf{K} & & \textbf{\si{\arcsecond}} & \textbf{mK} &\textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & \textbf{km s$^{-1}$} & & & \textbf{K km s$^{-1}$} \\ \hline 
  &&&&&\textbf{SO$_2$}&&\\ 
 \hline
 236.216 &16(1,15)-15(2,14) & 130.7 & -4.12 & 10 & 13 (3) & -1.4 & -2.4/-1.4 & 1.0 & 1.6& 0.8& 0.11 (0.02) \\ 
241.615 &5(2,4)-4(1,3) & 23.6 & -4.07 & 10 & 89 (3) & -0.3 & -7.1/2.6 & 1.0 & 1.6& 0.8& 0.88 (0.18) \\ 
254.280 &6(3,3)-6(2,4) & 41.4 & -3.94 & 10 & 23 (3) & 0.8 & -3.9/1.7 & 0.9 & 1.6& 0.8& 0.23 (0.05) \\ 
255.553 &4(3,1)-4(2,2) & 31.3 & -4.03 & 10 & 22 (4) & -1.1 & -2.9/0.8 & 0.9 & 1.6& 0.8& 0.24 (0.05) \\ 
256.246 &5(3,3)-5(2,4) & 35.9 & -3.97 & 10 & 21 (4) & -1.1 & -2.0/1.7 & 0.9 & 1.6& 0.8& 0.21 (0.04) \\ 
257.099 &7(3,5)-7(2,6) & 47.8 & -3.91 & 10 & 17 (3) & 0.8 & -3.8/2.6 & 0.9 & 1.7& 0.8& 0.22 (0.04) \\ 
271.529 &7(2,6)-6(1,5) & 35.5 & -3.96 & 9 & 47 (3) & -1.4 & -8.0/3.0 & 2.2 & 1.7& 0.8& 0.67 (0.13) \\ 
282.036 &6(2,4)-5(1,5) & 29.2 & -4.00 & 9 & 56 (3) & -1.2 & -5.5/3.0 & 2.1 & 1.8& 0.8& 0.74 (0.15) \\ 
283.464 &16(0,16)-15(1,15) & 121.0 & -3.57 & 9 & 29 (4) & -1.2 & -3.4/0.9 & 2.1 & 1.8& 0.8& 0.41 (0.08) \\ 
298.576 &9(2,8)-8(1,7) & 51.0 & -3.84 & 8 & 24 (3) & -1.0 & -3.0/3.0 & 2.0 & 1.9& 0.8& 0.34 (0.07) \\ 
313.279 &3(3,1)-2(2,0) & 27.6 & -3.47 & 8 & 14 (3) & 1.1 & -0.8/1.1 & 1.9 & 2.1& 0.9& 0.22 (0.04) \\ 
334.673 &8(2,6)-7(1,7) & 43.1 & -3.90 & 7 & 37 (4) & -0.6 & -4.2/1.2 & 1.8 & 2.3& 0.9& 0.49 (0.10) \\ 
\hline
 &&&&&\textbf{$^{34}$SO}&&\\ 
 \hline 
84.411 &2(2)-1(1) & 19.2 & -5.30 & 29 & 5 (1) & -0.2 & -1.6/1.2 & 1.4 & 1.0& 0.3& 0.03 (0.01) \\ 
97.715 &3(2)-2(1) & 9.1 & -4.96 & 25 & 75 (2) & 0.2 & -8.2/3.8 & 1.2 & 1.2& 0.4& 0.56 (0.11) \\ 
106.743 &2(3)-1(2) & 20.9 & -4.99 & 23 & 7 (2) & -1.8 & -2.9/-0.7 & 1.1 & 1.2& 0.4& 0.05 (0.01) \\ 
135.775 &4(3)-3(2) & 15.6 & -4.51 & 18 & 87 (4) & 0.9 & -6.9/3.5 & 0.9 & 1.2& 0.6& 0.56 (0.11) \\ 
155.506 &3(4)-2(3) & 28.4 & -4.39 & 16 & 25 (6) & 1.1 & -1.2/1.1 & 0.8 & 1.3& 0.6& 0.16 (0.03) \\ 
201.846 &4(5)-3(4) & 38.1 & -4.02 & 12 & 15 (3) & -0.9 & -3.2/2.6 & 1.2 & 1.5& 0.7& 0.19 (0.04) \\ 
211.013 &5(5)-4(4) & 43.5 & -3.94 & 12 & 14 (3) & 1.5 & -1.8/2.6 & 1.1 & 1.5& 0.8& 0.14 (0.03) \\ 
215.839 &6(5)-5(4) & 34.4 & -3.89 & 11 & 49 (3) & 0.4 & -6.1/3.7 & 1.1 & 1.5& 0.8& 0.47 (0.09) \\ 
\hline 
 &&&&&\textbf{$^{34}$SO$_2$}&&\\ 
 \hline 
133.471 &5(1,5)-4(0,4) & 15.6 & -4.68 & 18 & 12 (3) & 1.7 & 0.8/1.7 & 0.9 & 1.2& 0.5& 0.07 (0.01) \\ 
162.775 &7(1,7)-6(0,6) & 27.0 & -4.40 & 15 & 24 (6) & -1.0 & -1.0/2.6 & 0.7 & 1.3& 0.6& 0.19 (0.04) \\ 
\hline
\end{tabular}
\label{table:lines3}
\end{table*}



